A Temporal Type-2 Fuzzy System for Time-dependent Explainable Artificial Intelligence

Explainable Artificial Intelligence (XAI) is a paradigm that delivers transparent models and decisions, which are easy to understand, analyze, and augment by a non-technical audience. Fuzzy Logic Systems (FLS) based XAI can provide an explainable framework, while also modeling uncertainties present in real-world environments, which renders it suitable for applications where explainability is a requirement. However, most real-life processes are not characterized by high levels of uncertainties alone; they are inherently time-dependent as well, i.e., the processes change with time. In this work, we present novel Temporal Type-2 FLS Based Approach for time-dependent XAI (TXAI) systems, which can account for the likelihood of a measurement's occurrence in the time domain using (the measurement's) frequency of occurrence. In Temporal Type-2 Fuzzy Sets (TT2FSs), a four-dimensional (4D) time-dependent membership function is developed where relations are used to construct the inter-relations between the elements of the universe of discourse and its frequency of occurrence. The TXAI system manifested better classification prowess, with 10-fold test datasets, with a mean recall of 95.40\% than a standard XAI system (based on non-temporal general type-2 (GT2) fuzzy sets) that had a mean recall of 87.04\%. TXAI also performed significantly better than most non-explainable AI systems between 3.95\%, to 19.04\% improvement gain in mean recall. In addition, TXAI can also outline the most likely time-dependent trajectories using the frequency of occurrence values embedded in the TXAI model; viz. given a rule at a determined time interval, what will be the next most likely rule at a subsequent time interval. In this regard, the proposed TXAI system can have profound implications for delineating the evolution of real-life time-dependent processes, such as behavioural or biological processes.

==> Figures_texFiles_Used/Operators.tex <==
%--------------------------------------------------------------
%--------------------------------------------------------------
% Define block styles
%--------------------------------------------------------------
%--------------------------------------------------------------
\tikzstyle{decision} = [diamond, draw, fill=blue!20, 
    text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw,  
    text width=2.8cm, text centered, rounded corners, minimum height=1.5cm, fill= blue!30]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    minimum height=2em]
\tikzstyle{dotted_block} = [draw=black!30!white, line width=1pt, dash pattern=on 1pt off 4pt on 6pt off 4pt, inner ysep=1mm,inner xsep=1mm, rectangle, rounded corners ]
\tikzstyle{myarrows} = [draw=black,solid,line width=.5mm, ->]
\tikzstyle{dashedline} = [draw=black,dashed,line width=.5mm]
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
\begin{figure*}[!hbtp]
\centering
\begin{tikzpicture}
    \node (temp_MF_A) [block, fill= blue!30] {Temporal Membership Function};
    \node (temp_MF_B) [block, fill= blue!30, below of = temp_MF_A, node distance = 4cm] {Temporal Membership Function};
    \node (operator) [block, minimum height=2cm,right of = temp_MF_A, text width = 2cm, fill= green!30, node distance = 5cm, yshift= -2cm] {Operator};
    \node (relation) [block, right of = operator, text width = 2cm, fill= red!30, node distance = 6cm] {Relation};
    % Paths
    \draw[myarrows] ([yshift=0.15cm]temp_MF_A.east) -- node [xshift = .05cm, yshift=0.2cm] {\( \mu(x_A)\)} ++(1.5,0) |- ([yshift=.7cm]operator.west);
    \draw[myarrows] ([yshift=-0.15cm]temp_MF_A.east) -- node [xshift = .1cm, yshift=-0.3cm] {\(\mu(t_A)\)} ++(1.2,0) |- ([yshift=0.4cm]operator.west);
    \draw[myarrows] ([yshift=0.15cm]temp_MF_B.east) -- node [xshift = .1cm, yshift=0.2cm] {\( \mu(x_B)\)} ++(1.2,0) |- ([yshift=-.4cm]operator.west);
    \draw[myarrows] ([yshift=-0.15cm]temp_MF_B.east) -- node [xshift = .05cm, yshift=-0.3cm] { \(\mu(t_B)\)} ++(1.5,0) |- ([yshift=-0.7cm]operator.west);
    \draw[myarrows] ([yshift=0.4cm]operator.east) -- node [xshift = 0.05cm, yshift=0.4cm] {\( \mu(x_A) \) operator \(\mu(x_B)\)} ([yshift=0.4cm]relation.west);
    \draw[myarrows] ([yshift=-0.4cm]operator.east) -- node [xshift = 0.05cm, yshift=-0.3cm] {\(\mu(t_A)\) operator \(\mu(t_B)\)} ([yshift=-0.4cm]relation.west);
    \draw[myarrows] (relation.east) -- node [xshift = 1.5cm, yshift=0.3cm] {Temporal MF \( \mu_{A \text{operator} B}(x,t)\)}++(2,0);
\end{tikzpicture}
\caption{Crisp values of input data (x), and time (t), are first converted into membership fuzzy sets \(\mu(x) \) and \(\mu(t) \) that are then transformed into a temporal membership fuzzy set using relations (such as Mamdani relation) on \(\mu(x) \) and \(\mu(t) \).}
\label{Fig:TemporalOperator}
\end{figure*}
